Improving the Efficiency of VVC using Partitioning of Reference Frames

In response to the growing demand for high-quality videos, Versatile Video Coding (VVC) was released in 2020, building on the hybrid coding architecture of its predecessor, HEVC, achieving about 50% bitrate reduction for the same visual quality. It introduces more flexible block partitioning, enhancing compression efficiency at the cost of increased encoding complexity. To make efficient use of VVC in practical applications, optimization is essential. VVenC, an optimized open-source VVC encoder, introduces multiple presets to address the trade-off between compression efficiency and encoder complexity. Although an optimized set of encoding tools has been selected for each preset, the rate-distortion (RD) search space in the encoder presets still poses a challenge for efficient encoder implementations. In this paper, we propose Early Termination using Reference Frames (ETRF), which improves the trade-off between encoding efficiency and time complexity and positions itself as a new preset between medium and fast presets. The CTU partitioning map of the reference frames in lower temporal layers is employed to accelerate the encoding of frames in higher temporal layers. The results show a reduction in the encoding time of around 21% compared to the medium preset. Specifically, for videos with high spatial and temporal complexities, which typically require longer encoding times, the proposed method achieves a better trade-off between bitrate savings and encoding time compared to the fast preset.

==> extra.tex <==
%Bitmovin employs Dynamic Adaptive Streaming over HTTP (DASH) standardized by Moving Picture Experts Group (MPEG), known as MPEG-DASH \ref{}. 


%There are numerous ways to reduce the compression complexity of VVC. Here we focus on the block based complextiy reduction methods for Intra and Inter frames.
%In the recent works for Intra frame block based complexity reduction 

 %Wang et al. use a two stage machine learning based model predict the partitioning type and hence reduce the RD search space. Tisseer
%There are various works to reduce the complexity of block based partitioning structure in VVC. The research works mainly focus on reducing the search space of block partitioning of Intra frame and Inter frame.    


%Some of the techniques focus solely on reducing the encoding complexity of the Intra frame~\cite{shang2023fast,wang2023fsvm,chen2023speed,song2024fast}, which has only spatial redundancy. Others focus on reducing the encoding complexity of Intra- and inter-frames, which includes spatial and temporal redundancies~\cite{jiang2023extreme,kuang2022unified,lin2024efficient,liu2022light}. Although the encoding usually has very few Intra-frames, their encoding time is larger than Inter-frames~\cite{bossen2021vvc}, which motivates researchers to focus on reducing the complexity of intra-frames using all intra profiles. 

%\textcolor{red}{Read abstract and conclusion of papers and your understanding of works}

%In the real-world scenario where streaming applications are used, a video is encoded in multiple bitrates. Multirate techniques are deployed to make the flow more efficient by reducing the Rate-Distortion Cost searches also known as the search space. In this direction, most works are done on HEVC~\cite{sullivan2012overview}, the predecessor of VVC. 
%\textcolor{red}{Write review of Schroeder, the story is incomplete without this review.}

%Schroeder et al.~\cite{schroeder2015block} used the CU structure information of low QP videos, i.e., high-quality videos, also known as reference representations,  to limit the depth of high QP videos, i.e., low-quality videos, also known as the dependent representations. The dependent CU depth is limited to the maximum CU depth of the reference representation. Amirpour et al.~\cite{amirpour2020fast} extended the work to bound the dependent representation between two reference representations. 
%\textcolor{red}{Hadi did a double bound work before Cetinkaya add here}
%Cetinkaya et al.~\cite{cetinkaya2020fame} used the lowest quality video as the reference representation and applied CNNs to predict the depths of dependent representations of high-quality videos. The acceleration of the process is achieved by encoding the higher quality video with lower quality video in parallel. Amirpour et al.~\cite{amirpour2021towards} searched for an optimal reference representation to bound the dependent resolutions. The author experimented with multiple-quality videos and generated different modes for each quality to reduce the encoding time of dependent representations.  Cetinkaya et al.~\cite{cetinkaya2021fast} extended their work to multiresolution by using the CU structure information of the lowest resolution. The author designated the highest bitrate in the lowest resolution as the reference representation to reduce the encoding time for all higher resolutions. Recently, Memon et al.~\cite{menon2023emes} demonstrated multiple encoding schemes for x.265, real-time HEVC encoder. In the VVenC domain, there is only one work Liu et al.~\cite{liu2023preparing}, who applied the efficiency improvement based on multirate encoding. In multirate approaches there is a dependent representation whose encoding time is reduced using the reference representation. The idea behind the multirate is that dependent representations have similarities with the reference representations and hence can help in accelerating the search for the optimal Rate-Distortion Cost. 




%Several studies aim to reduce the RD optimization burden for Inter-frames by leveraging temporal and spatial features. Kuang et al. use historical data from previously checked partitions to predict the current CU's depth for both Intra- and Inter-frames. Shang et al. limit the number of modes (SKIP, Inter, affine, merge, Intra) evaluated for a CU block by considering the area and prediction modes of neighboring CUs. Li et al. employ a multi decision-tree approach for partitioning decisions to optimize the RD search space for Inter-frames. Liu et al. propose a CNN model that splits a CTU into an $8/times8$ grid, using depth information within each grid for optimization. Peng et al. develop a partition homogeneity map (PHM) to bypass RD cost searches for Inter-frames. Jiang et al. utilize an extreme learning machine (ELM) algorithm for early split decisions. Lin et al. adopt a supervised contrastive learning algorithm to predict partitioning patterns. However, these studies implement their algorithms on the VVC Test Model (VTM), which is an unoptimized reference software for VVC.
